Ultra-low-power second-order nonlinear optics on a chip

Second-order nonlinear optical processes are used to convert light from one wavelength to another and to generate quantum entanglement. Creating chip-scale devices to more efficiently realize and control these interactions greatly increases the reach of photonics. Optical crystals and guided wave devices made from lithium niobate and potassium titanyl phosphate are typically used to realize second-order processes but face significant drawbacks in scalability, power, and tailorability when compared to emerging integrated photonic systems. Silicon or silicon nitride integrated photonic circuits enhance and control the third-order optical nonlinearity by confining light in dispersion-engineered waveguides and resonators. An analogous platform for second-order nonlinear optics remains an outstanding challenge in photonics. It would enable stronger interactions at lower power and reduce the number of competing nonlinear processes that emerge. Here we demonstrate efficient frequency doubling and parametric oscillation in a thin-film lithium niobate photonic circuit. Our device combines recent progress on periodically poled thin-film lithium niobate waveguidesand low-loss microresonators. Here we realize efficient >10% second-harmonic generation and parametric oscillation with microwatts of optical power using a periodically-poled thin-film lithium niobate microresonator. The operating regimes of this system are controlled using the relative detuning of the intracavity resonances. During nondegenerate oscillation, the emission wavelength is tuned over terahertz by varying the pump frequency by 100's of megahertz. We observe highly-enhanced effective third-order nonlinearities caused by cascaded second-order processes resulting in parametric oscillation. These resonant second-order nonlinear circuits will form a crucial part of the emerging nonlinear and quantum photonics platforms.

==> methods.tex <==
\section*{Methods}

\subsection{Fabrication}
We fabricate all devices with X-cut thin-film lithium niobate-on-insulator (LNOI) wafers. The material consists of a 500 nm film of LN bonded to a 2 $\mu$m layer of silicon dioxide on top of an LN handle wafer. 

We pattern the optical devices using electron beam lithography (JEOL 6300-FS, 100-kV) and transfer the design to the LN via Argon ion milling. The etch depth is 300 nm, which leaves a 200 nm slab of LN beneath the waveguide. We deposit 700 nm of PECVD silicon dioxide at a temperature of 350 $ ^{\circ}$C as cladding. 

 We perform the periodic poling step before waveguide fabrication. For periodic poling, we use electron-beam evaporated Cr electrodes with an electron beam lithography-based liftoff process and apply high-voltage pulses similar to Nagy \textit{et al.} \cite{Nagy2019} to invert the crystal domains. Upon completion of the poling, we remove the electrodes. 

Chip edge facet preparation is done using a DISCO DFL7340 laser saw. High energy pulses are focused into the substrate to create a periodic array of damage locations, which act as nucleation sites for crack propagation and result in a uniform and smooth cleave. 

\subsection{Experimental Setup}
We characterize fabricated devices in a simplified experimental setup shown in Figure \ref{fig:2}a. In the FH input path, we use SMF-28 fibers. 5\% of the laser light (Santec TSL-550, 1480-1630 nm) goes into a Mach-Zehnder interferometer (MZI) with an FSR of 67.7 MHz used to calibrate the relative wavelength during laser wavelength sweeps (not shown in \ref{fig:2}a). 95\% of the light goes to erbium-doped fiber amplifier (EDFA) with a fixed output power of 250~mW followed by a variable optical attenuator. Next, the light passes through a fiber polarization controller (FPC), and we tap 5\% of it just before the input lensed fiber for power calibration with a power meter (Newport 918D-IR-OD3R). The light then couples to the chip facet through an SMF-28 lensed fiber.

In the SH path, we use a Velocity TLB-6700 laser that operates in the 765-781 nm range. This entire path uses 780HP fiber to maintain single-mode operation. A 5\% tap outcouples part of the light an MZI with an FSR of 39.9 MHz to calibrate laser wavelength sweeps (not shown in \ref{fig:2}a).  A variable optical attenuator controls the remaining laser power, and we control the polarization with an FPC. 5\% of the light goes to a power meter (Newport 918D-SL-OD3R) for input power calibration, and we focus the rest of it on the chip facet through a 780HP lensed fiber.

Once the light exits the output edge facet of the chip, we collect it into a lensed SMF-28 fiber, similar to the one used in the FH input path. We outcouple the light into free space and demultiplex with a 1000 nm short pass dichroic mirror. After the dichroic mirror, SH and FH paths are additionally filtered to ensure no cross talk, and we detect SH and FH light with avalanche photodiodes (Thorlabs APD410A and Thorlabs APD410, respectively). Variable optical attenuators are used before the APDs to avoid saturation. We split 50\% of the FH light into an optical spectrum analyzer (OSA, Yokogawa AQ6370D) for spectrally-resolved measurements of the OPO.

We use different, but similar, devices on the same chip for the SHG and OPO experiments. The chip sits directly on a thermo-electric cooler for temperature adjustment.

\subsection{OPO Characterization}
We characterize all of the optical resonances that take part in the optical parametric oscillation using linear spectroscopy at powers substantially below nonlinear effects. For these measurements, we sweep the wavelength of tunable lasers in the FH and SH bands and fit the transmission dips with lorentzian lineshapes. We determine the total and intrinsic quality factors of the second harmonic mode to be $Q_{B,0} = 0.88 \times 10^{6}$ and $Q_{B,0}^{\text{(i)}} = 1.5 \times 10^{6}$, respectively. We find the quality factors of the OPO signal modes corresponding to the curve in \ref{fig:2}a to be: $Q_{A,m} = 0.68 \times 10^{6}$, $Q_{A,m}^{\text{(i)}} = 0.8 \times 10^{6}$, $Q_{A,-m} = 0.94 \times 10^{6}$, $Q_{A,-m}^{\text{(i)}} = 1.5 \times 10^{6}$. We perform an independent second harmonic generation measurements to determine if the FH and SH modes are under or overcoupled. The analysis of transmission lineshapes as a function of pump power confirms that all modes are undercoupled. From the determined threshold of 73 $\mu$W we deduce a coupling rate $|g_{0,-mm}|$ of 150 kHz which is close to the simulated value of 186 kHz.

We measure the input fiber-to-chip coupling with an independent transmission measurement using 780HP lensed fibers at the input and the output chip edges. We assume the input and output coupling is identical, an assumption based on experience with multiple devices on the chip used for the experiment, and find the input edge coupling efficiency to be 13\%. We extract the output fiber-to-chip coupling efficiency at the OPO wavelength by fitting the data in Fig. \ref{fig:3}a to $\eta_{\text{FH}}P_{\text{out}}$ using equation \ref{eqn:PoutOPOwithDisorder_main}. We infer $\eta_{FH}$ = 37\% coupling efficiency, which we confirm with an independent transmission measurement.

\subsection{SHG Characterization}
We characterize the modes contributing to the second harmonic generation in an analogous way to the OPO. From the Lorentzian fits at low power we find quality factors of $Q_{B,0} = 0.82 \times 10^{6}$, $Q_{B,0}^{\text{(i)}} = 1.2 \times 10^{6}$, $Q_{A,0} = 0.75 \times 10^{6}$, and $Q_{A,0}^{\text{(i)}} = 1.2 \times 10^{6}$. Moreover, we use a method for fitting nonlinear lineshapes at high power, as mentioned in the main text. For this purpose, we solve equations \ref{eqn:steadystate_A0} and \ref{eqn:steadystate_BK} numerically and fit the resulting curves as a function of detuning to the data. We use the ten lineshapes at the pump power between 80 and 620 $\mu$W, which allows us to observe changes due to the second-order nonlinearities but avoid the effects of the cascaded OPO. From this procedure we find average $Q_{A,0} = 0.74 \times 10^{6}$, and $Q_{A,0}^{\text{(i)}} = 1.2 \times 10^{6}$ and standard deviation of less than 4\% which agrees with the low power fit. From fitting nonlinear lineshapes, we also extract the coupling rate $|g_{0,00}|$ to be about 130 kHz, which agrees with our theoretical prediction of 170 kHz. In the main text, we use averaged values to plot the theoretical lineshapes and only vary the modal detuning to account for small temperature fluctuations. For the SHG device, we calibrate the fiber-to-chip coupling efficiency at the FH and SH by fitting the nonlinear transmission and response data. We find the coupling efficiencies to be to be 26\% and 11\%, respectively. 

We calculate the theoretical relationship between the pump power, SHG power, and SHG efficiency by numerically solving equations \ref{eqn:steadystate_A0} and \ref{eqn:steadystate_BK} for zero detuning. For the solid lines plotted in Figure \ref{fig:4}a, we use quality factors and the nonlinear coupling rate from the measurements described in the previous paragraph.

\subsection{Resolving OPO Lines}
We use an OSA (Yokogawa AQ370D) to characterize the frequency content of the OPO output spectrum as a function of pump laser detuning. With a constant pump power, we repeatedly sweep the laser wavelength across the SH resonance and record the SH and FH response with APDs (see section Experimental Setup). A portion of the generated FH light is detected by the OSA operating in zero-span mode with a 0.1 nm filter bandwidth, which is less than the approximately 0.135 nm free spectral range of the FH modes. We step the center wavelength of the OSA across a 40 nm span with a 50\% overlap in OSA filter spans. We record the detected power on the OSA synchronously with the APD detector voltages for each wavelength step. Repeated laser sweeps with different OSA filter center wavelengths produce a map of the OPO frequency content as a function of laser detuning shown in \ref{fig:3}b. 

To characterize the cascaded parametric oscillations as shown in \ref{fig:4}d, we first find every potential OPO line's precise location ($\omega_m$) by performing a broad sweep of the FH pump laser and record the resonance frequencies. We then proceeded with the measurement in an identical fashion to the standard OPO, but with the 0.1 nm wide OSA filters placed precisely at the FH mode locations without any overlap between filters.

%

\subsection{Coupled Mode Theory Equations}

The Hamiltonian of the system is used to find the equations of motion in the rotating frame. 
\begin{eqnarray}
\frac{\textrm{d}}{\textrm{d}t} A_m &=& -\frac{\kappa_{A,m}}{2} A_m - 2i \sum_{k n} g_{k,nm} A_n^\ast B_k e^{-i\delta_{k,nm}t} - \nonumber\\&&~~~~ \sqrt{\kappa^{\text{(e)}}_{A,m}}F_m e^{-i(\omega_L - \omega_m)t} \label{eqn:dAdt}\\
\frac{\textrm{d}}{\textrm{d}t}  B_k &=& -\frac{\kappa_{B,k}}{2} B_k - i  \sum_{m n} g^\ast_{k,nm} A_m A_n e^{+i\delta_{k,nm}t} -\nonumber\\&&~~~~ \sqrt{\kappa^{\text{(e)}}_{B,k}}G_k e^{-i(\Omega_L - \Omega_k)t} \label{eqn:dBdt},
\end{eqnarray}
with $\delta_{k,nm}=\Omega_k -\omega_n -\omega_m$. $A_m$ is the fundamental field amplitude at $\omega_m$, and $B_k$ is the second harmonic field amplitude at $\Omega_k$.


\subsection{Parametric Oscillation Theory}

We consider the case where the SH modes are driven at frequency $\Omega_L$ and the $A$ modes are not excited and calculate the stability criterion for the $A$ modes based on equation (\ref{eqn:dBdt}):
\begin{eqnarray}
\frac{\textrm{d}}{\textrm{d}t}  B_0 &=& -\frac{\kappa_{B,0}}{2} B_0 -  \sqrt{\kappa^{\text{(e)}}_{B,0}}G_0 e^{-i(\Omega_L - \Omega_0)t} \label{eqn:opo_dBdt}.
\end{eqnarray}
We go into a rotating frame $B_0 = \Tilde{B}_0 e^{-i\Delta t}$ with frequency $\Delta = \Omega_L - \Omega_0$ defined as the detuning between the laser drive and the $B$  mode, which we can solve in steady-state to obtain:
\begin{eqnarray}
\Tilde{B}_0 = \frac{ \sqrt{\kappa^{\text{(e)}}_{B,0}}G_0}{i\Delta - {\kappa_{B,0}}/{2}}.\label{eqn:opo_B0_driven}
\end{eqnarray}
We now consider two $A$ modes at frequencies $\omega_m$ and $\omega_{-m}$ which are coupled by the intracavity population of $B_0$. Their coupling leads to a pair of equations
\begin{eqnarray}
\frac{\textrm{d}}{\textrm{d}t}  A_m &=& -\frac{\kappa_{A,m}}{2} A_m - 2 i g_{0,-mm} A_{-m}^\ast B_0 e^{-i\delta_{0,-mm}t} \nonumber %
\\
\frac{\textrm{d}}{\textrm{d}t}  A^\ast_{-m} &=& -\frac{\kappa_{A,-m}}{2} A_{-m}^\ast + 2i g^\ast_{0,-mm} A_{m} B^\ast_0 e^{i\delta_{0,-mm}t} \nonumber%
\end{eqnarray}
which become unstable for sufficiently large $|B_0|$. To see this note that $\delta_{0,-mm} = (\Omega_0 - 2\omega_0) - \zeta_2 m^2$ allowing us to move into a rotating frame with 
\begin{eqnarray}
A_m = \Tilde{A}_m \exp\left( -i\frac{\Delta+\mu-\zeta_2 m^2}{2}t \right)
\end{eqnarray}
where $\mu\equiv\Omega_0 - 2\omega_0$ is the \emph{modal detuning} between the driven SH and closest FH mode, which in our experiment is set by tuning the temperature.
In this frame, the equations become time-independent, and we obtain the stability criterion (assuming $\kappa_{\pm m}$ are equal for simplicity):
\begin{eqnarray}
16|g_{0,-mm}|^2 |B_0|^2 \ge \left( \Delta + \mu - \zeta_2 m^2 \right)^2 + \left(\kappa_{A,m}\right)^2.\label{eqn:opo_stab_crit_1}
\end{eqnarray}
To relate this to the input photon flux at the SH frequency $\Omega_0$, we replace $B_0$ using eqn.~(\ref{eqn:opo_B0_driven}), to obtain
\begin{eqnarray}
16|g_{0,-mm}|^2&& |G_0|^2 \kappa^{\text{(e)}}_{B,0} \ge 
\left( \Delta^2 + \left({\kappa_{B,0}}/{2} \right)^2 \right)\times\nonumber\\&&~~~
\left(
\left( \Delta + \mu - \zeta_2 m^2 \right)^2 + \left({\kappa_{A,m}} \right)^2\right).\label{eqn:opo_stab_crit_2}
\end{eqnarray}
We can see from here that the lowest degenerate oscillation threshold can be achieved when $\mu=0$ and $\Delta=0$:
\begin{eqnarray}
4|g_{0,-mm}|^2 |G_0|^2 \kappa^{\text{(e)}}_{B,0} &\ge& 
\left({\kappa_{B,0}}/{2} \right)^2
 \left({\kappa_{A,m}}/{2} \right)^2~\text{or,}\\
 P_\text{th,0} &=&\frac{\hbar \Omega_0}{64 |g_{0,00}|^2}\frac{\kappa^{2}_{B,0} \kappa^{2}_{A,0} }{\kappa^{\text{(e)}}_{B,0}}.
\end{eqnarray}
More generally, the OPO will oscillate first in the mode $m$ for which $ P_{\text{th},m}$ is the lowest, where
\begin{eqnarray}
P_{\text{th},m} &=& \frac{\hbar \Omega_0}{16 |g_{0,-mm}|^2}\frac{1 }{\kappa^{\text{(e)}}_{B,0}} \left( \Delta^2 + \left({\kappa_{B,0}}/{2} \right)^2 \right)\times\nonumber\\&&
\left(
\left( \Delta + \mu - \zeta_2 m^2 \right)^2 + \left({\kappa_{A,m}} \right)^2\right). \label{eqn:opo_P_th_l}
\end{eqnarray}
Here we've assumed again that the losses for the $\pm m$ modes are equal. Equation~(\ref{eqn:opo_P_th_l}) shows that we can use the modal detuning $\mu$ and the driving detuning $\Delta$ to select which modes reach threshold first and oscillate as the power is increased. Assuming that $g_{0,-mm}$ does not change significantly with the mode number, we see that for on-resonant driving $\Delta=0$, a minimum threshold can be achieved when $\mu=\zeta_2 m^2$, as long as $\mu$ and $\zeta_2$ have the same sign. In our case, the waveguide has normal dispersion, so $\zeta_2$ is negative, and we have roughly $\zeta_2/2\pi= -100~\textrm{kHz}$. The relation $m \approx \sqrt{\mu/\zeta_2}$ shows that the mode number selected is very sensitive to the modal detuning (set by temperature) which makes the degenerate oscillation mode challenging to obtain in a system with a large resonator and therefore very small $\zeta_2$ mode-spacing dispersion parameter. 

Interestingly, if the modal detuning $\mu$ is held constant while the pump detuning $\Delta$ is swept, the oscillation threshold can select very different modes $m$ with only small changes in $\Delta$.  When the laser is nearly resonant with $\Omega_0$, so $\Delta$ is small compared to the $B$ mode linewidth, the first term in parenthesis in eqn~(\ref{eqn:opo_P_th_l}) is minimized and does not vary strongly with detuning, while the second term is minimized whenever $\Delta+\mu \approx \zeta_2 m^2$.  This means that with a fixed laser input power, sweeping the laser across the second harmonic mode causes oscillation at very different mode numbers and explains the spectrum in figure~\ref{fig:3}b. For example, if we set $\Delta \ll \kappa_{B,0}$, we would obtain an approximate equation for the oscillating mode index (which should be rounded to obtain an integer, and requires $\mu+\Delta$ to have the same sign as $\zeta_2$):
\begin{eqnarray}
m \approx \sqrt{\frac{\mu+\Delta}{\zeta_2 }}
\label{eqn:muCondition}
\end{eqnarray}

For the real device, we observe disorder in the loss rates for different signal modes, which can result from fabrication imperfections or coupler dispersion. We can account for that in our threshold calculation
\begin{eqnarray}
P_{\text{th},m} &=& \frac{\hbar \Omega_0}{16 |g_{0,-mm}|^2}\frac{1 }{\kappa^{\text{(e)}}_{B,0}} \left( \Delta^2 + \left({\kappa_{B,0}}/{2} \right)^2 \right)\times\nonumber\\&&
\left(
\left( \Delta + \mu - \zeta_2 m^2 \right)^2 + \kappa_{A,m} \kappa_{A,-m}\right). \label{eqn:opo_P_th_l_disorder}
\end{eqnarray}
To obtain a relation for the OPO power output, we solve equations (\ref{eqn:dAdt}) - (\ref{eqn:dBdt}) for specific modes in steady-state. For the zero detuning of the pump mode $\Delta = 0$ and assuming $\mu = \zeta_2 m^2$, we have:
\begin{eqnarray}
A_m &=& 
\cfrac{4ig_{0,-mm} A_{-m}^{\ast} B_{0}}{\kappa_{A,m}}
\label{eqn:Am}\\
B_0 &=& 
\cfrac{2ig^{\ast}_{0,-mm}A_m A_{-m} + \sqrt{\kappa_{B,0}^{\text{(e)}}} G_{0} }{\kappa_{B,0}/2}
\label{eqn:Bk}.
\end{eqnarray}
Now, if we note that the oscillating amplitudes and coupling rate are complex $A_m = |A_m|\text{exp}(i\theta_m)$, $g_{k,00} = |g_{k,00}|\text{exp}(i\varphi)$, we can substitute equation (\ref{eqn:Am}) to (\ref{eqn:Bk}) and obtain
\begin{eqnarray}\cfrac{\kappa_{A,m} \kappa_{B,0} }{8i|g_{0,-mm}|^2} \cfrac{|A_{m}|}{|A_{-m}|} -2i|A_{m}||A_{-m}| + \nonumber\\
\cfrac{\sqrt{\kappa_{B,0}^{\text{(e)}}} }{|g_{0,-mm}|} G_{0} e^{i(\varphi - \theta_m - \theta_{-m})} = 0.
\label{eqn:ImCondition}
\end{eqnarray}
This requires the exponential $\text{exp}(i(\varphi - \theta_m - \theta_{-m}))$ to be purely imaginary, $\varphi - \theta_m - \theta_{-m} = \pi/2 + d\cdot\pi$, where $d\in\mathbb{Z}$. This phase relation shows that the sum of the phases of the OPO output are locked to the phase of the pump. As a result, we can use equation (\ref{eqn:Am}) to find that
\begin{eqnarray}
\cfrac{|A_m|}{|A_{-m}|} = \sqrt{\cfrac{\kappa_{A,-m}}{\kappa_{A,m}}},
\label{eqn:AmAnrelation}
\end{eqnarray}
and solve equation (\ref{eqn:ImCondition}) for the photon flux of both signal modes of the OPO:
\begin{eqnarray}
|A_{m}|^2 = \sqrt{\cfrac{\kappa_{A,-m}}{\kappa_{A,m}}} \cfrac{\sqrt{\kappa_{B,0}^{\text{(e)}}} G_{0}}{2|g_{0,-mm}|}
-\cfrac{\kappa_{B,0} \kappa_{A,m}}{16 |g_{0,-mm}|^2}
\label{eqn:AmModSq}
\\
|A_{-m}|^2 = \sqrt{\cfrac{\kappa_{A,m}}{\kappa_{A,-m}}} \cfrac{\sqrt{\kappa_{B,0}^{\text{(e)}}} G_{0}}{2|g_{0,-mm}|}
-\cfrac{\kappa_{B,0} \kappa_{A,-m}}{16 |g_{0,-mm}|^2}.
\label{eqn:AnModSq}
\end{eqnarray}
To analyze the total output power of the OPO in experiment, we sum over the power of two signal modes
\begin{eqnarray}
P_{\text{out}} = 
\cfrac{4\eta_{B,0}}{\Omega_{0}}
\left(
\eta_{A,m}\omega_{m}+ 
\eta_{A,-m}\omega_{-m}
\right)
\times \nonumber \\
P_{\text{th,m}}
\left(
\sqrt{\cfrac{P_{\text{B,0}}}{P_{\text{th,m}}}} - 1
\right),
\label{eqn:PoutOPOwithDisorder}
\end{eqnarray}
with $\eta_k=\kappa^{\text{(e)}}_{k,0}/\kappa_{k,0}$ for $k=A,B$ being the cavity-waveguide coupling efficiency. $P_{\text{B,0}}$ is the pump power of the SH mode and $P_{\text{th,m}}$ is a generalized OPO threshold, which includes disorder in the total loss rates of fundamental modes:
\begin{eqnarray}
P_{\text{th,m}} &=&
\cfrac{\hbar \Omega_{0}}{64|g_{0,-mm}|^2} \cfrac{\kappa_{B,0}^2\kappa_{A,m}\kappa_{A,-m}}{\kappa_{B,0}^{\text{(e)}}} = 
\nonumber\\&&
\cfrac{\hbar \Omega_{0}}{16 \eta_B} \cfrac{\sqrt{ \kappa_{A,m} \kappa_{A,-m}}}{C_{0,m} },
\label{eqn:PthresholdWithDisorder}
\end{eqnarray}
where $C_{0,m} \equiv 4|g_{0,-mm}|^2/\left(\sqrt{\kappa_{A,m}\kappa_{A,-m}}\kappa_{B,0}\right)$ is the vacuum cooperativity for $m^{\text{th}}$ pair of signal modes. Note that this relation agrees with equation (\ref{eqn:opo_P_th_l_disorder}) for the case of modal and laser detuning optimized for $m^{\text{th} }$ OPO sideband.

\subsection{Second Harmonic Generation Efficiency}


Starting from the coupled mode equations~(\ref{eqn:dAdt}) and (\ref{eqn:dBdt}), we now assume that only $A_0$ is excited, i.e., we are driving the mode at $\omega_0$ and all other mode FH amplitudes are $0$:
\begin{eqnarray}
\frac{\textrm{d}}{\textrm{d}t}  A_0 &=& - \frac{\kappa_{A,i}}{2} A_0 - 2 i  \sum_{k} g_{k,00} A_0^\ast B_k e^{-i\delta_{k,00}t} \nonumber \\&&~~~~~~~~~ - \sqrt{\kappa^{\text{(e)}}_{A,0}}F_0 e^{-i(\omega_L - \omega_0)t} \\
\frac{\textrm{d}}{\textrm{d}t}  B_k &=& -\frac{\kappa_{B,k}}{2} B_k - i g^{\ast}_{k,00} A_0^2 e^{+i\delta_{k, 00}t}.
\end{eqnarray}
To solve these equations, we go into a frame that rotates with the laser detuning frequency $\delta =\omega_L - \omega_0$, so $ A_0 = \Tilde A_0 e^{-i\delta t}$, $B_k = \Tilde B_k e^{-i(2\delta-\delta_{k, 0 0})t} = \Tilde B_k e^{-i(2\omega_L - \Omega_k)t}$:
\begin{eqnarray}
\frac{\textrm{d}}{\textrm{d}t}  \Tilde A_0 &=& \left(i\delta-\frac{\kappa_{A,i}}{2}\right) \Tilde A_0 - 2 i  \sum_{k} g_{k,00} \Tilde A_0^\ast \Tilde B_k - \nonumber\\&&~~~~~~~~~ \sqrt{\kappa^{\text{(e)}}_{A,0}}F_0 \\
\frac{\textrm{d}}{\textrm{d}t}  \Tilde B_k &=& \left(i(2\omega_L-\Omega_k)-\frac{\kappa_{B,k}}{2}\right) \Tilde B_{k} - i  g_{k,00}^\ast \Tilde A_0^2 .
\end{eqnarray}
We can solve these in steady state to obtain:
\begin{eqnarray}
\Tilde B_k = \frac{ig^{\ast}_{k,00} \Tilde A_0^2}{i(2\omega_L-\Omega_k)-\frac{\kappa_{B,k}}{2}}\label{eqn:steadystate_BK}
\end{eqnarray}
\begin{eqnarray}
0 &=& \left( i\delta - \frac{\kappa_{A,0}}{2}\right) \Tilde A_0 +  \sum_{k} \frac{2 |g_{k,00}|^2 |\Tilde A_0|^2}{i(2\omega_L - \Omega_k)-\frac{\kappa_{B,k}}{2}} \Tilde A_0 -\nonumber\\&&~~~~~~~~~ \sqrt{\kappa^{\text{(e)}}_{A,0}} F_0 \label{eqn:steadystate_A0}
\end{eqnarray}
There are a couple of interesting things to note about the last equation. Note that each SH mode at $\Omega_k$ contributes effective nonlinear loss and detuning terms to the FH mode at $\omega_0$:
\begin{eqnarray}
\text{Detuning:}~&& - \sum_k \frac{2(2\omega_L - \Omega_k)}{(2\omega_L - \Omega_k)^2 + \left(\frac{\kappa_{B,k}}{2}\right)^2} g_{k,00}^2 |A_0|^2 \label{eqn:2photon_detuning}\\
\text{Loss:}~&& \sum_k \frac{2\kappa_{B,k}}{(2\omega_L - \Omega_k)^2 + \left(\frac{\kappa_{B,k}}{2}\right)^2} g_{k,00}^2 |A_0|^2 \label{eqn:2photon_loss}
\end{eqnarray}
For large $2\omega_L - \Omega_{k} \gg \kappa_b$, we see an effect which is primarily a frequency shift and looks much like a $\chi^{(3)}$ cavity frequency shift.%

From here on, we assume that only one SH mode $(k=0)$ is significantly excited. The photons generated at the $B_0$ mode frequency are emitted from the device generating a photon flux $|G_{\text{out},0}|^2$ at the SH frequency where $G_{\text{out},0} = \sqrt{\kappa^{\text{(e)}}_{B,0}} \Tilde B_0$. To find $\Tilde B_0$, we need to calculate $\Tilde A_0$ (eqn~\ref{eqn:steadystate_BK}), which is given implicitly by 
\begin{eqnarray}
0 &=& \left( i\delta - \frac{\kappa_{A,0}}{2}\right) \Tilde A_0 +  \frac{ 2|g_{0,00}|^2 |\Tilde A_0|^2}{i(2\omega_L - \Omega_0)-\frac{\kappa_{B,0}}{2}} \Tilde A_0 -\nonumber\\&&~~~~~~~~~ \sqrt{\kappa^{\text{(e)}}_{A,0}} F_0. \label{eqn:steadystate_A0_single_mode}
\end{eqnarray}
For the fits shown in the paper, this equation was solved numerically. Here we assume $\delta=0$ and approximate the solutions in two limits, 1) the low-power limit where the first term is dominant, and 2) the high-power limit where the second term is dominant. The cross-over between these two limits occurs at
\begin{eqnarray}
2 C_0 n_A^{(0)} = 1
\end{eqnarray}
where $C_0 = 4g_{0,00}^2/\kappa_{A,0}\kappa_{B,0}$ is a cooperativity parameter and $n_A^{(0)} = {4 \kappa^{\text{(e)}}_{A,0}|F_0|^2 }/{{\kappa_{A,0}^2}} $ is the number of intracavity photons which would be excited in the absence of nonlinearity. 
Solving the above equation in the two limits gives us 
\begin{eqnarray}
|\Tilde A_0|^2 = n_A^{(0)}, \textrm{and}~~~~
|\Tilde A_0|^2 = \left(\frac{n_A^{(0)}}{4 C_0^2}\right)^{1/3}\nonumber
\end{eqnarray}
for the low- and high-power limits respectively. We define the second harmonic generation power efficiency 
\begin{eqnarray}
\eta_{\text{SHG}} \equiv \frac{P_\text{out}}{P_\text{in}} = \frac{2|G_{\text{out},0}|^2}{|F_0|^2},
\end{eqnarray}
which after some manipulation, can be written in terms of $|\Tilde A_0|^2$:
\begin{eqnarray}
\eta_{\text{SHG}} &=& \frac{8 \eta_A\eta_B C_0}{n_A^{(0)}} |\Tilde A_0|^4\nonumber\\
&=& \begin{cases}
      8 \eta_A \eta_B C_0 n^{(0)}_A & \text{low power}\\
      \cfrac{4 \eta_A \eta_B}{(2n^{(0)}_A C_0)^{1/3}}& \text{high power}
    \end{cases}       
\end{eqnarray}
It is apparent that at low power, the efficiency increases linearly, but is then saturated at high power. This can be understood from an impedance matching perspective. As the pump power is increased, the FH cavity resonance senses a two-photon loss proportional to $4|g_{0,00} \Tilde A_0|^2/\kappa_{B,0}$ (see eqn.~\ref{eqn:2photon_loss}). As this loss starts to exceed the cavity linewidth, its effective coupling rate to the waveguide is reduced, preventing input light from coupling efficiently into the cavity to be frequency-doubled. At very high power, the efficiency actually begins to go down as  $P^{-1/3}$. The model assumes that only the $\Tilde B_0$ and $\Tilde A_0$ modes are excited. As we saw in the case of a directly driven OPO, at sufficiently large $\Tilde B_0$, $\Tilde A_{\pm m}$ start to oscillate, which causes this model to break down and the system to go into cascaded optical parametric oscillation. 



\subsection*{Cascaded Optical Parametric Oscillation}
 
Consider the same driving as in the previous section, where a laser drive at the fundamental with frequency $\omega_L$ excites $\Tilde A_0$ and generates an intracavity population in the second harmonic mode $\Tilde B_0$. From the section on the oscillation threshold, we know that at a sufficiently value of $|\Tilde B_0|$, the equations of motion for mode amplitudes $\Tilde A_{\pm m}$ become unstable and set of oscillations, with a threshold condition given by an equation very similar to eqn.~(\ref{eqn:opo_stab_crit_1}):
\begin{eqnarray}
16|g_{0,-mm}|^2 |\Tilde B_0|^2  \geq \left(2\delta +\mu - {\zeta_2}m^2\right)^2 +  {\kappa_{A,m}}{\kappa_{A,-m}}.\nonumber \label{eqn:copo_stab_crit_3}
\end{eqnarray}
%
%
%
We call this a cascaded OPO, since a cascade of two back-to-back $\chi^{(2)}$ processes leads to a an effective $\chi^{(3)}$ four-wave mixing process. It is clear from the oscillation condition that the threshold is highly detuning-dependent, and also depends on the dispersion parameter $\zeta_2$. In our case, $\zeta_2/2\pi\approx -100~\textrm{kHz}$ and so the oscillation threshold is lower with the laser tuned to the red side ($\delta<0$) when the modal detuning $\mu \approx 0$.

\subsection{Nonlinear Coupling Rate}\label{sec:g_theory}

We derive the nonlinear coupling rate from the interaction energy density in the three-wave mixing process. Given the electric field distribution $\m E{} = (E^x,E^y,E^z)$ The  interaction energy density  is given by:
\begin{eqnarray}
U_{\chi^{(2)}} =
\cfrac{\varepsilon_{0}}{3} \sum_{\alpha \beta \gamma} \chi_{\alpha \beta \gamma}^{(2)} {E}^{\alpha} {E}^{\beta} {E}^{\gamma},
\label{eqn:nlInteractionE}
\end{eqnarray}
each of the three waves can be expressed using spatial complex amplitudes $\m Em, \m En, \m Ek$ as follows:
\begin{eqnarray}
\m{E}{} &=& 
A_m \m {E}m e^{-i\omega_m t} +
A_n \m{E}n e^{-i\omega_n t} + B_k\m{E}k e^{-i\Omega_k t} \nonumber\\&&~~~~~~~~~~ + \textrm{h.c.}
\label{eqn:Ealpha}
\end{eqnarray}
To calculate the nonlinear coupling rate we focus on three specific modes in the sum and evaluate equation \ref{eqn:nlInteractionE} by averaging away the rapidly rotating terms. It selects only energy-conserving terms of the sum. Since the second-order nonlinear tensor has a full permutation symmetry, for the non-degenerate we find that
\begin{eqnarray}
U^{k,nm}_{\chi^{(2)}} &=&
2\varepsilon_{0} \sum_{\alpha \beta \gamma}
\chi^{(2)}_{\alpha \beta \gamma}
\left(
{E}^{\alpha\ast}_{k} {E}^{\beta}_{m} {E}^{\gamma}_{n} B_k^{\ast} A_m A_n  + \text{h.c.} \right)
= \nonumber \\&&
2\varepsilon_{0}
\left(
\m{E}k^{\ast} \bar{\bar{\chi}}^{(2)}:\m{E}{m} \m{E}{n} B_k^{\ast} A_m A_n  + \text{h.c.}
\right).
\label{eqn:nlInteractionE_2}
\end{eqnarray}
Integrating over this energy density gives us the total energy of the system, which we use to derive the equations of motion (\ref{eqn:dAdt}) and (\ref{eqn:dBdt}). We choose normalization of the modal field $\m {E}{k}$ so that the total energy corresponding to an amplitude $A_k$ is $\hbar \omega_k |A_k|^2$. More precisely, given unitless field profiles $\m ei$ (with $\textrm{max} (\m ei) = 1$), we introduce normalization factors $N_i$, defined by $\m Ei = N_i \m ei$. The energy condition then fixes these normalization factors as
\begin{eqnarray}
N_i &=& \sqrt{\cfrac{\hbar \omega_i}{2\int \m ei^\ast \bar{\bar{\varepsilon}}(\m r{})\m ei dV}} \nonumber\\
 &=& \sqrt{\cfrac{\hbar \omega_i}{2\varepsilon_0 L \int  \m ei^\ast \bar{\bar{\varepsilon}}_r(\m r{})\m ei dA}}\nonumber\\
 &=& \sqrt{\cfrac{\hbar \omega_i}{2\varepsilon_0 L \bar n_i^2}}\frac{1}{\sqrt{\mathcal{A}_i}}
\label{eqn:nlInteractionE_norm}
\end{eqnarray}
Here, we introduced the effective mode area for each mode as $\mathcal{A}_i = \int_{A} |\m{e}{i}|^2 dA$, and define the average index as $ \bar n_i^2=\int  \m ei^\ast \bar{\bar{\varepsilon}}_r(\m r{})\m ei dA /\mathcal{A}_i$. To find the energy, we integrate equation \ref{eqn:nlInteractionE_2} over the mode volume. We account for a partially-poled racetrack resonator by introducing the poled length fraction $\lambda$ as a ratio of the poled region to the total resonator length $L$. The final expression for the nonlinear coupling rate is given by:
\begin{eqnarray}
g_{k,nm} = \cfrac{\lambda}{\sqrt{2} \pi} \sqrt{\cfrac{\hbar\omega_m\omega_n\Omega_k}{\varepsilon_0 L \bar n_k^2 \bar n_m^2 \bar n_n^2}} \cfrac{\mathcal{O}}{\sqrt{\mathcal{A}_m \mathcal{A}_n \mathcal{A}_k}},
\label{eqn:nlCouplingRate}
\end{eqnarray}
where $\mathcal{O}$ represents the mode overlap integral over the waveguide cross section area
\begin{eqnarray}
\mathcal{O} = 
\int_{A} \m{e}{k}^{\ast} \bar{\bar{\chi}}^{(2)}:
\m{e}{m} \m{e}{n} dA.
\label{eqn:overlapIntegral}
\end{eqnarray}
For our numerical waveguide calculations we use a finite-element mode solver (COMSOL).

\subsection{Numerical Simulations of Dynamics}

We numerically integrate the coupled mode differential equations (\ref{eqn:dAdt}) and (\ref{eqn:dBdt}) to understand how the transmission spectra change when the system starts to oscillate and how disorder affects the emission spectra. We integrate the coupled mode equations with with $181$ $A$ modes and $31$ $B$ modes for $600$ nanoseconds which is sufficiently long for the system to stabilize. We use the measured parameters from the SHG experiment for the $\omega_0$ and $\Omega_0$ modes, and assume that the other modes are spaced by the measured FSR (which agrees with the theory prediction) and have the same quality factors. The resulting spectra for are shown in Extended Figure Fig. \ref{fig:FigSI2}. We then perform the same simulation but with the quality factors and detunings of the other modes now having disorder (normally distributed fluctuations of total $Q$ and mode frequency) on the order of $1\%$ (Fig. \ref{fig:FigSI3}) and $10\%$ (Fig. \ref{fig:FigSI4}) of the cavity linewidth. 

 

==> sec_theory_dont_edit_this.tex <==

\subsection{Coupled Mode Theory Equations}

The Hamiltonian of the system is used to find the equations of motion in the rotating frame. 
\begin{eqnarray}
\frac{\textrm{d}}{\textrm{d}t} A_m &=& -\frac{\kappa_{A,m}}{2} A_m - 2i \sum_{k n} g_{k,nm} A_n^\ast B_k e^{-i\delta_{k,nm}t} - \nonumber\\&&~~~~ \sqrt{\kappa^{\text{(e)}}_{A,m}}F_m e^{-i(\omega_L - \omega_m)t} \label{eqn:dAdt}\\
\frac{\textrm{d}}{\textrm{d}t}  B_k &=& -\frac{\kappa_{B,k}}{2} B_k - i  \sum_{m n} g^\ast_{k,nm} A_m A_n e^{+i\delta_{k,nm}t} -\nonumber\\&&~~~~ \sqrt{\kappa^{\text{(e)}}_{B,k}}G_k e^{-i(\Omega_L - \Omega_k)t} \label{eqn:dBdt},
\end{eqnarray}
with $\delta_{k,nm}=\Omega_k -\omega_n -\omega_m$. $A_m$ is the fundamental field amplitude at $\omega_m$, and $B_k$ is the second harmonic field amplitude at $\Omega_k$.


\subsection{Parametric Oscillation Theory}

We consider the case where the SH modes are driven at frequency $\Omega_L$ and the $A$ modes are not excited and calculate the stability criterion for the $A$ modes based on equation (\ref{eqn:dBdt}):
\begin{eqnarray}
\frac{\textrm{d}}{\textrm{d}t}  B_0 &=& -\frac{\kappa_{B,0}}{2} B_0 -  \sqrt{\kappa^{\text{(e)}}_{B,0}}G_0 e^{-i(\Omega_L - \Omega_0)t} \label{eqn:opo_dBdt}.
\end{eqnarray}
We go into a rotating frame $B_0 = \Tilde{B}_0 e^{-i\Delta t}$ with frequency $\Delta = \Omega_L - \Omega_0$ defined as the detuning between the laser drive and the $B$  mode, which we can solve in steady-state to obtain:
\begin{eqnarray}
\Tilde{B}_0 = \frac{ \sqrt{\kappa^{\text{(e)}}_{B,0}}G_0}{i\Delta - {\kappa_{B,0}}/{2}}.\label{eqn:opo_B0_driven}
\end{eqnarray}
We now consider two $A$ modes at frequencies $\omega_m$ and $\omega_{-m}$ which are coupled by the intracavity population of $B_0$. Their coupling leads to a pair of equations
\begin{eqnarray}
\frac{\textrm{d}}{\textrm{d}t}  A_m &=& -\frac{\kappa_{A,m}}{2} A_m - 2 i g_{0,-mm} A_{-m}^\ast B_0 e^{-i\delta_{0,-mm}t} \nonumber %
\\
\frac{\textrm{d}}{\textrm{d}t}  A^\ast_{-m} &=& -\frac{\kappa_{A,-m}}{2} A_{-m}^\ast + 2i g^\ast_{0,-mm} A_{m} B^\ast_0 e^{i\delta_{0,-mm}t} \nonumber%
\end{eqnarray}
which become unstable for sufficiently large $|B_0|$. To see this note that $\delta_{0,-mm} = (\Omega_0 - 2\omega_0) - \zeta_2 m^2$ allowing us to move into a rotating frame with 
\begin{eqnarray}
A_m = \Tilde{A}_m \exp\left( -i\frac{\Delta+\mu-\zeta_2 m^2}{2}t \right)
\end{eqnarray}
where $\mu\equiv\Omega_0 - 2\omega_0$ is the \emph{modal detuning} between the driven SH and closest FH mode, which in our experiment is set by tuning the temperature.
In this frame, the equations become time-independent, and we obtain the stability criterion (assuming $\kappa_{\pm m}$ are equal for simplicity):
\begin{eqnarray}
16|g_{0,-mm}|^2 |B_0|^2 \ge \left( \Delta + \mu - \zeta_2 m^2 \right)^2 + \left(\kappa_{A,m}\right)^2.\label{eqn:opo_stab_crit_1}
\end{eqnarray}
To relate this to the input photon flux at the SH frequency $\Omega_0$, we replace $B_0$ using eqn.~(\ref{eqn:opo_B0_driven}), to obtain
\begin{eqnarray}
16|g_{0,-mm}|^2&& |G_0|^2 \kappa^{\text{(e)}}_{B,0} \ge 
\left( \Delta^2 + \left({\kappa_{B,0}}/{2} \right)^2 \right)\times\nonumber\\&&~~~
\left(
\left( \Delta + \mu - \zeta_2 m^2 \right)^2 + \left({\kappa_{A,m}} \right)^2\right).\label{eqn:opo_stab_crit_2}
\end{eqnarray}
We can see from here that the lowest degenerate oscillation threshold can be achieved when $\mu=0$ and $\Delta=0$:
\begin{eqnarray}
4|g_{0,-mm}|^2 |G_0|^2 \kappa^{\text{(e)}}_{B,0} &\ge& 
\left({\kappa_{B,0}}/{2} \right)^2
 \left({\kappa_{A,m}}/{2} \right)^2~\text{or,}\\
 P_\text{th,0} &=&\frac{\hbar \Omega_0}{64 |g_{0,00}|^2}\frac{\kappa^{2}_{B,0} \kappa^{2}_{A,0} }{\kappa^{\text{(e)}}_{B,0}}.
\end{eqnarray}
More generally, the OPO will oscillate first in the mode $m$ for which $ P_{\text{th},m}$ is the lowest, where
\begin{eqnarray}
P_{\text{th},m} &=& \frac{\hbar \Omega_0}{16 |g_{0,-mm}|^2}\frac{1 }{\kappa^{\text{(e)}}_{B,0}} \left( \Delta^2 + \left({\kappa_{B,0}}/{2} \right)^2 \right)\times\nonumber\\&&
\left(
\left( \Delta + \mu - \zeta_2 m^2 \right)^2 + \left({\kappa_{A,m}} \right)^2\right). \label{eqn:opo_P_th_l}
\end{eqnarray}
Here we've assumed again that the losses for the $\pm m$ modes are equal. Equation~(\ref{eqn:opo_P_th_l}) shows that we can use the modal detuning $\mu$ and the driving detuning $\Delta$ to select which modes reach threshold first and oscillate as the power is increased. Assuming that $g_{0,-mm}$ does not change significantly with the mode number, we see that for on-resonant driving $\Delta=0$, a minimum threshold can be achieved when $\mu=\zeta_2 m^2$, as long as $\mu$ and $\zeta_2$ have the same sign. In our case, the waveguide has normal dispersion, so $\zeta_2$ is negative, and we have roughly $\zeta_2/2\pi= -100~\textrm{kHz}$. The relation $m \approx \sqrt{\mu/\zeta_2}$ shows that the mode number selected is very sensitive to the modal detuning (set by temperature) which makes the degenerate oscillation mode challenging to obtain in a system with a large resonator and therefore very small $\zeta_2$ mode-spacing dispersion parameter. 

Interestingly, if the modal detuning $\mu$ is held constant while the pump detuning $\Delta$ is swept, the oscillation threshold can select very different modes $m$ with only small changes in $\Delta$.  When the laser is nearly resonant with $\Omega_0$, so $\Delta$ is small compared to the $B$ mode linewidth, the first term in parenthesis in eqn~(\ref{eqn:opo_P_th_l}) is minimized and does not vary strongly with detuning, while the second term is minimized whenever $\Delta+\mu \approx \zeta_2 m^2$.  This means that with a fixed laser input power, sweeping the laser across the second harmonic mode causes oscillation at very different mode numbers and explains the spectrum in figure~\ref{fig:3}b. For example, if we set $\Delta \ll \kappa_{B,0}$, we would obtain an approximate equation for the oscillating mode index (which should be rounded to obtain an integer, and requires $\mu+\Delta$ to have the same sign as $\zeta_2$):
\begin{eqnarray}
m \approx \sqrt{\frac{\mu+\Delta}{\zeta_2 }}
\label{eqn:muCondition}
\end{eqnarray}

For the real device, we observe disorder in the loss rates for different signal modes, which can result from fabrication imperfections or coupler dispersion. We can account for that in our threshold calculation
\begin{eqnarray}
P_{\text{th},m} &=& \frac{\hbar \Omega_0}{16 |g_{0,-mm}|^2}\frac{1 }{\kappa^{\text{(e)}}_{B,0}} \left( \Delta^2 + \left({\kappa_{B,0}}/{2} \right)^2 \right)\times\nonumber\\&&
\left(
\left( \Delta + \mu - \zeta_2 m^2 \right)^2 + \kappa_{A,m} \kappa_{A,-m}\right). \label{eqn:opo_P_th_l_disorder}
\end{eqnarray}
To obtain a relation for the OPO power output, we solve equations (\ref{eqn:dAdt}) - (\ref{eqn:dBdt}) for specific modes in steady-state. For the zero detuning of the pump mode $\Delta = 0$ and assuming $\mu = \zeta_2 m^2$, we have:
\begin{eqnarray}
A_m &=& 
\cfrac{4ig_{0,-mm} A_{-m}^{\ast} B_{0}}{\kappa_{A,m}}
\label{eqn:Am}\\
B_0 &=& 
\cfrac{2ig^{\ast}_{0,-mm}A_m A_{-m} + \sqrt{\kappa_{B,0}^{\text{(e)}}} G_{0} }{\kappa_{B,0}/2}
\label{eqn:Bk}.
\end{eqnarray}
Now, if we note that the oscillating amplitudes and coupling rate are complex $A_m = |A_m|\text{exp}(i\theta_m)$, $g_{k,00} = |g_{k,00}|\text{exp}(i\varphi)$, we can substitute equation (\ref{eqn:Am}) to (\ref{eqn:Bk}) and obtain
\begin{eqnarray}\cfrac{\kappa_{A,m} \kappa_{B,0} }{8i|g_{0,-mm}|^2} \cfrac{|A_{m}|}{|A_{-m}|} -2i|A_{m}||A_{-m}| + \nonumber\\
\cfrac{\sqrt{\kappa_{B,0}^{\text{(e)}}} }{|g_{0,-mm}|} G_{0} e^{i(\varphi - \theta_m - \theta_{-m})} = 0.
\label{eqn:ImCondition}
\end{eqnarray}
This requires the exponential $\text{exp}(i(\varphi - \theta_m - \theta_{-m}))$ to be purely imaginary, $\varphi - \theta_m - \theta_{-m} = \pi/2 + d\cdot\pi$, where $d\in\mathbb{Z}$. This phase relation shows that the sum of the phases of the OPO output are locked to the phase of the pump. As a result, we can use equation (\ref{eqn:Am}) to find that
\begin{eqnarray}
\cfrac{|A_m|}{|A_{-m}|} = \sqrt{\cfrac{\kappa_{A,-m}}{\kappa_{A,m}}},
\label{eqn:AmAnrelation}
\end{eqnarray}
and solve equation (\ref{eqn:ImCondition}) for the photon flux of both signal modes of the OPO:
\begin{eqnarray}
|A_{m}|^2 = \sqrt{\cfrac{\kappa_{A,-m}}{\kappa_{A,m}}} \cfrac{\sqrt{\kappa_{B,0}^{\text{(e)}}} G_{0}}{2|g_{0,-mm}|}
-\cfrac{\kappa_{B,0} \kappa_{A,m}}{16 |g_{0,-mm}|^2}
\label{eqn:AmModSq}
\\
|A_{-m}|^2 = \sqrt{\cfrac{\kappa_{A,m}}{\kappa_{A,-m}}} \cfrac{\sqrt{\kappa_{B,0}^{\text{(e)}}} G_{0}}{2|g_{0,-mm}|}
-\cfrac{\kappa_{B,0} \kappa_{A,-m}}{16 |g_{0,-mm}|^2}.
\label{eqn:AnModSq}
\end{eqnarray}
To analyze the total output power of the OPO in experiment, we sum over the power of two signal modes
\begin{eqnarray}
P_{\text{out}} = 
\cfrac{4\eta_{B,0}}{\Omega_{0}}
\left(
\eta_{A,m}\omega_{m}+ 
\eta_{A,-m}\omega_{-m}
\right)
\times \nonumber \\
P_{\text{th,m}}
\left(
\sqrt{\cfrac{P_{\text{B,0}}}{P_{\text{th,m}}}} - 1
\right),
\label{eqn:PoutOPOwithDisorder}
\end{eqnarray}
with $\eta_k=\kappa^{\text{(e)}}_{k,0}/\kappa_{k,0}$ for $k=A,B$ being the cavity-waveguide coupling efficiency. $P_{\text{B,0}}$ is the pump power of the SH mode and $P_{\text{th,m}}$ is a generalized OPO threshold, which includes disorder in the total loss rates of fundamental modes:
\begin{eqnarray}
P_{\text{th,m}} &=&
\cfrac{\hbar \Omega_{0}}{64|g_{0,-mm}|^2} \cfrac{\kappa_{B,0}^2\kappa_{A,m}\kappa_{A,-m}}{\kappa_{B,0}^{\text{(e)}}} = 
\nonumber\\&&
\cfrac{\hbar \Omega_{0}}{16 \eta_B} \cfrac{\sqrt{ \kappa_{A,m} \kappa_{A,-m}}}{C_{0,m} },
\label{eqn:PthresholdWithDisorder}
\end{eqnarray}
where $C_{0,m} \equiv 4|g_{0,-mm}|^2/\left(\sqrt{\kappa_{A,m}\kappa_{A,-m}}\kappa_{B,0}\right)$ is the vacuum cooperativity for $m^{\text{th}}$ pair of signal modes. Note that this relation agrees with equation (\ref{eqn:opo_P_th_l_disorder}) for the case of modal and laser detuning optimized for $m^{\text{th} }$ OPO sideband.

\subsection{Second Harmonic Generation Efficiency}


Starting from the coupled mode equations~(\ref{eqn:dAdt}) and (\ref{eqn:dBdt}), we now assume that only $A_0$ is excited, i.e., we are driving the mode at $\omega_0$ and all other mode FH amplitudes are $0$:
\begin{eqnarray}
\frac{\textrm{d}}{\textrm{d}t}  A_0 &=& - \frac{\kappa_{A,i}}{2} A_0 - 2 i  \sum_{k} g_{k,00} A_0^\ast B_k e^{-i\delta_{k,00}t} \nonumber \\&&~~~~~~~~~ - \sqrt{\kappa^{\text{(e)}}_{A,0}}F_0 e^{-i(\omega_L - \omega_0)t} \\
\frac{\textrm{d}}{\textrm{d}t}  B_k &=& -\frac{\kappa_{B,k}}{2} B_k - i g^{\ast}_{k,00} A_0^2 e^{+i\delta_{k, 00}t}.
\end{eqnarray}
To solve these equations, we go into a frame that rotates with the laser detuning frequency $\delta =\omega_L - \omega_0$, so $ A_0 = \Tilde A_0 e^{-i\delta t}$, $B_k = \Tilde B_k e^{-i(2\delta-\delta_{k, 0 0})t} = \Tilde B_k e^{-i(2\omega_L - \Omega_k)t}$:
\begin{eqnarray}
\frac{\textrm{d}}{\textrm{d}t}  \Tilde A_0 &=& \left(i\delta-\frac{\kappa_{A,i}}{2}\right) \Tilde A_0 - 2 i  \sum_{k} g_{k,00} \Tilde A_0^\ast \Tilde B_k - \nonumber\\&&~~~~~~~~~ \sqrt{\kappa^{\text{(e)}}_{A,0}}F_0 \\
\frac{\textrm{d}}{\textrm{d}t}  \Tilde B_k &=& \left(i(2\omega_L-\Omega_k)-\frac{\kappa_{B,k}}{2}\right) \Tilde B_{k} - i  g_{k,00}^\ast \Tilde A_0^2 .
\end{eqnarray}
We can solve these in steady state to obtain:
\begin{eqnarray}
\Tilde B_k = \frac{ig^{\ast}_{k,00} \Tilde A_0^2}{i(2\omega_L-\Omega_k)-\frac{\kappa_{B,k}}{2}}\label{eqn:steadystate_BK}
\end{eqnarray}
\begin{eqnarray}
0 &=& \left( i\delta - \frac{\kappa_{A,0}}{2}\right) \Tilde A_0 +  \sum_{k} \frac{2 |g_{k,00}|^2 |\Tilde A_0|^2}{i(2\omega_L - \Omega_k)-\frac{\kappa_{B,k}}{2}} \Tilde A_0 -\nonumber\\&&~~~~~~~~~ \sqrt{\kappa^{\text{(e)}}_{A,0}} F_0 \label{eqn:steadystate_A0}
\end{eqnarray}
There are a couple of interesting things to note about the last equation. Note that each SH mode at $\Omega_k$ contributes effective nonlinear loss and detuning terms to the FH mode at $\omega_0$:
\begin{eqnarray}
\text{Detuning:}~&& - \sum_k \frac{2(2\omega_L - \Omega_k)}{(2\omega_L - \Omega_k)^2 + \left(\frac{\kappa_{B,k}}{2}\right)^2} g_{k,00}^2 |A_0|^2 \label{eqn:2photon_detuning}\\
\text{Loss:}~&& \sum_k \frac{2\kappa_{B,k}}{(2\omega_L - \Omega_k)^2 + \left(\frac{\kappa_{B,k}}{2}\right)^2} g_{k,00}^2 |A_0|^2 \label{eqn:2photon_loss}
\end{eqnarray}
For large $2\omega_L - \Omega_{k} \gg \kappa_b$, we see an effect which is primarily a frequency shift and looks much like a $\chi^{(3)}$ cavity frequency shift.%

From here on, we assume that only one SH mode $(k=0)$ is significantly excited. The photons generated at the $B_0$ mode frequency are emitted from the device generating a photon flux $|G_{\text{out},0}|^2$ at the SH frequency where $G_{\text{out},0} = \sqrt{\kappa^{\text{(e)}}_{B,0}} \Tilde B_0$. To find $\Tilde B_0$, we need to calculate $\Tilde A_0$ (eqn~\ref{eqn:steadystate_BK}), which is given implicitly by 
\begin{eqnarray}
0 &=& \left( i\delta - \frac{\kappa_{A,0}}{2}\right) \Tilde A_0 +  \frac{ 2|g_{0,00}|^2 |\Tilde A_0|^2}{i(2\omega_L - \Omega_0)-\frac{\kappa_{B,0}}{2}} \Tilde A_0 -\nonumber\\&&~~~~~~~~~ \sqrt{\kappa^{\text{(e)}}_{A,0}} F_0. \label{eqn:steadystate_A0_single_mode}
\end{eqnarray}
For the fits shown in the paper, this equation was solved numerically. Here we assume $\delta=0$ and approximate the solutions in two limits, 1) the low-power limit where the first term is dominant, and 2) the high-power limit where the second term is dominant. The cross-over between these two limits occurs at
\begin{eqnarray}
2 C_0 n_A^{(0)} = 1
\end{eqnarray}
where $C_0 = 4g_{0,00}^2/\kappa_{A,0}\kappa_{B,0}$ is a cooperativity parameter and $n_A^{(0)} = {4 \kappa^{\text{(e)}}_{A,0}|F_0|^2 }/{{\kappa_{A,0}^2}} $ is the number of intracavity photons which would be excited in the absence of nonlinearity. 
Solving the above equation in the two limits gives us 
\begin{eqnarray}
|\Tilde A_0|^2 = n_A^{(0)}, \textrm{and}~~~~
|\Tilde A_0|^2 = \left(\frac{n_A^{(0)}}{4 C_0^2}\right)^{1/3}\nonumber
\end{eqnarray}
for the low- and high-power limits respectively. We define the second harmonic generation power efficiency 
\begin{eqnarray}
\eta_{\text{SHG}} \equiv \frac{P_\text{out}}{P_\text{in}} = \frac{2|G_{\text{out},0}|^2}{|F_0|^2},
\end{eqnarray}
which after some manipulation, can be written in terms of $|\Tilde A_0|^2$:
\begin{eqnarray}
\eta_{\text{SHG}} &=& \frac{8 \eta_A\eta_B C_0}{n_A^{(0)}} |\Tilde A_0|^4\nonumber\\
&=& \begin{cases}
      8 \eta_A \eta_B C_0 n^{(0)}_A & \text{low power}\\
      \cfrac{4 \eta_A \eta_B}{(2n^{(0)}_A C_0)^{1/3}}& \text{high power}
    \end{cases}       
\end{eqnarray}
It is apparent that at low power, the efficiency increases linearly, but is then saturated at high power. This can be understood from an impedance matching perspective. As the pump power is increased, the FH cavity resonance senses a two-photon loss proportional to $4|g_{0,00} \Tilde A_0|^2/\kappa_{B,0}$ (see eqn.~\ref{eqn:2photon_loss}). As this loss starts to exceed the cavity linewidth, its effective coupling rate to the waveguide is reduced, preventing input light from coupling efficiently into the cavity to be frequency-doubled. At very high power, the efficiency actually begins to go down as  $P^{-1/3}$. The model assumes that only the $\Tilde B_0$ and $\Tilde A_0$ modes are excited. As we saw in the case of a directly driven OPO, at sufficiently large $\Tilde B_0$, $\Tilde A_{\pm m}$ start to oscillate, which causes this model to break down and the system to go into cascaded optical parametric oscillation. 



\subsection*{Cascaded Optical Parametric Oscillation}
 
Consider the same driving as in the previous section, where a laser drive at the fundamental with frequency $\omega_L$ excites $\Tilde A_0$ and generates an intracavity population in the second harmonic mode $\Tilde B_0$. From the section on the oscillation threshold, we know that at a sufficiently value of $|\Tilde B_0|$, the equations of motion for mode amplitudes $\Tilde A_{\pm m}$ become unstable and set of oscillations, with a threshold condition given by an equation very similar to eqn.~(\ref{eqn:opo_stab_crit_1}):
\begin{eqnarray}
16|g_{0,-mm}|^2 |\Tilde B_0|^2  \geq \left(2\delta +\mu - {\zeta_2}m^2\right)^2 +  {\kappa_{A,m}}{\kappa_{A,-m}}.\nonumber \label{eqn:copo_stab_crit_3}
\end{eqnarray}
%
%
%
We call this a cascaded OPO, since a cascade of two back-to-back $\chi^{(2)}$ processes leads to a an effective $\chi^{(3)}$ four-wave mixing process. It is clear from the oscillation condition that the threshold is highly detuning-dependent, and also depends on the dispersion parameter $\zeta_2$. In our case, $\zeta_2/2\pi\approx -100~\textrm{kHz}$ and so the oscillation threshold is lower with the laser tuned to the red side ($\delta<0$) when the modal detuning $\mu \approx 0$.

\subsection{Nonlinear Coupling Rate}\label{sec:g_theory}

We derive the nonlinear coupling rate from the interaction energy density in the three-wave mixing process. Given the electric field distribution $\m E{} = (E^x,E^y,E^z)$ The  interaction energy density  is given by:
\begin{eqnarray}
U_{\chi^{(2)}} =
\cfrac{\varepsilon_{0}}{3} \sum_{\alpha \beta \gamma} \chi_{\alpha \beta \gamma}^{(2)} {E}^{\alpha} {E}^{\beta} {E}^{\gamma},
\label{eqn:nlInteractionE}
\end{eqnarray}
each of the three waves can be expressed using spatial complex amplitudes $\m Em, \m En, \m Ek$ as follows:
\begin{eqnarray}
\m{E}{} &=& 
A_m \m {E}m e^{-i\omega_m t} +
A_n \m{E}n e^{-i\omega_n t} + B_k\m{E}k e^{-i\Omega_k t} \nonumber\\&&~~~~~~~~~~ + \textrm{h.c.}
\label{eqn:Ealpha}
\end{eqnarray}
To calculate the nonlinear coupling rate we focus on three specific modes in the sum and evaluate equation \ref{eqn:nlInteractionE} by averaging away the rapidly rotating terms. It selects only energy-conserving terms of the sum. Since the second-order nonlinear tensor has a full permutation symmetry, for the non-degenerate we find that
\begin{eqnarray}
U^{k,nm}_{\chi^{(2)}} &=&
2\varepsilon_{0} \sum_{\alpha \beta \gamma}
\chi^{(2)}_{\alpha \beta \gamma}
\left(
{E}^{\alpha\ast}_{k} {E}^{\beta}_{m} {E}^{\gamma}_{n} B_k^{\ast} A_m A_n  + \text{h.c.} \right)
= \nonumber \\&&
2\varepsilon_{0}
\left(
\m{E}k^{\ast} \bar{\bar{\chi}}^{(2)}:\m{E}{m} \m{E}{n} B_k^{\ast} A_m A_n  + \text{h.c.}
\right).
\label{eqn:nlInteractionE_2}
\end{eqnarray}
Integrating over this energy density gives us the total energy of the system, which we use to derive the equations of motion (\ref{eqn:dAdt}) and (\ref{eqn:dBdt}). We choose normalization of the modal field $\m {E}{k}$ so that the total energy corresponding to an amplitude $A_k$ is $\hbar \omega_k |A_k|^2$. More precisely, given unitless field profiles $\m ei$ (with $\textrm{max} (\m ei) = 1$), we introduce normalization factors $N_i$, defined by $\m Ei = N_i \m ei$. The energy condition then fixes these normalization factors as
\begin{eqnarray}
N_i &=& \sqrt{\cfrac{\hbar \omega_i}{2\int \m ei^\ast \bar{\bar{\varepsilon}}(\m r{})\m ei dV}} \nonumber\\
 &=& \sqrt{\cfrac{\hbar \omega_i}{2\varepsilon_0 L \int  \m ei^\ast \bar{\bar{\varepsilon}}_r(\m r{})\m ei dA}}\nonumber\\
 &=& \sqrt{\cfrac{\hbar \omega_i}{2\varepsilon_0 L \bar n_i^2}}\frac{1}{\sqrt{\mathcal{A}_i}}
\label{eqn:nlInteractionE_norm}
\end{eqnarray}
Here, we introduced the effective mode area for each mode as $\mathcal{A}_i = \int_{A} |\m{e}{i}|^2 dA$, and define the average index as $ \bar n_i^2=\int  \m ei^\ast \bar{\bar{\varepsilon}}_r(\m r{})\m ei dA /\mathcal{A}_i$. To find the energy, we integrate equation \ref{eqn:nlInteractionE_2} over the mode volume. We account for a partially-poled racetrack resonator by introducing the poled length fraction $\lambda$ as a ratio of the poled region to the total resonator length $L$. The final expression for the nonlinear coupling rate is given by:
\begin{eqnarray}
g_{k,nm} = \cfrac{\lambda}{\sqrt{2} \pi} \sqrt{\cfrac{\hbar\omega_m\omega_n\Omega_k}{\varepsilon_0 L \bar n_k^2 \bar n_m^2 \bar n_n^2}} \cfrac{\mathcal{O}}{\sqrt{\mathcal{A}_m \mathcal{A}_n \mathcal{A}_k}},
\label{eqn:nlCouplingRate}
\end{eqnarray}
where $\mathcal{O}$ represents the mode overlap integral over the waveguide cross section area
\begin{eqnarray}
\mathcal{O} = 
\int_{A} \m{e}{k}^{\ast} \bar{\bar{\chi}}^{(2)}:
\m{e}{m} \m{e}{n} dA.
\label{eqn:overlapIntegral}
\end{eqnarray}
For our numerical waveguide calculations we use a finite-element mode solver (COMSOL).

\subsection{Numerical Simulations of Dynamics}

We numerically integrate the coupled mode differential equations (\ref{eqn:dAdt}) and (\ref{eqn:dBdt}) to understand how the transmission spectra change when the system starts to oscillate and how disorder affects the emission spectra. We integrate the coupled mode equations with with $181$ $A$ modes and $31$ $B$ modes for $600$ nanoseconds which is sufficiently long for the system to stabilize. We use the measured parameters from the SHG experiment for the $\omega_0$ and $\Omega_0$ modes, and assume that the other modes are spaced by the measured FSR (which agrees with the theory prediction) and have the same quality factors. The resulting spectra for are shown in Extended Figure Fig. \ref{fig:FigSI2}. We then perform the same simulation but with the quality factors and detunings of the other modes now having disorder (normally distributed fluctuations of total $Q$ and mode frequency) on the order of $1\%$ (Fig. \ref{fig:FigSI3}) and $10\%$ (Fig. \ref{fig:FigSI4}) of the cavity linewidth. 


